Locally Regular and Efficient Tests in Non-Regular Semiparametric Models

This paper considers hypothesis testing in semiparametric models which may be non-regular. I show that C($\alpha$) style tests are locally regular under mild conditions, including in cases where locally regular estimators do not exist, such as models which are (semiparametrically) weakly identified. I characterise the appropriate limit experiment in which to study local (asymptotic) optimality of tests in the non-regular case and generalise classical power bounds to this case. I give conditions under which these power bounds are attained by the proposed C($\alpha$) style tests. The application of the theory to a single index model and an instrumental variables model is worked out in detail.

==> size_1_exponential.tex <==

\begin{tabular}{l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Homoskedastic} & \multicolumn{3}{c}{Heteroskedastic} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
$n$ & $f_1$ & $f_2$ & $f_3$ & $f_1$ & $f_2$ & $f_3$\\
\midrule\multicolumn{7}{l}{$\psi_{n, \theta_0}$}\\
\midrule
400 & 6.04 & 5.86 & 5.28 & 5.38 & 5.42 & 4.80\\
600 & 5.50 & 5.38 & 5.10 & 5.82 & 5.48 & 5.32\\
800 & 5.10 & 5.14 & 5.40 & 5.62 & 5.82 & 5.28\\
\midrule\multicolumn{7}{l}{Wald}\\\midrule
\addlinespace
400 & 15.10 & 19.24 & 13.62 & 17.68 & 20.38 & 14.60\\
600 & 12.20 & 16.64 & 13.00 & 14.46 & 19.38 & 14.54\\
800 & 10.16 & 15.22 & 12.90 & 12.06 & 19.48 & 13.52\\
\bottomrule
\end{tabular}


==> size_1_logistic.tex <==

\begin{tabular}{l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}l*{6}{>{\raggedleft\arraybackslash}p{3em}}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Homoskedastic} & \multicolumn{3}{c}{Heteroskedastic} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
$n$ & $f_1$ & $f_2$ & $f_3$ & $f_1$ & $f_2$ & $f_3$\\
\midrule\multicolumn{7}{l}{$\psi_{n, \theta_0}$}\\
\midrule
400 & 6.24 & 5.72 & 5.62 & 6.06 & 5.68 & 5.24\\
600 & 5.70 & 5.54 & 5.62 & 5.44 & 5.32 & 5.24\\
800 & 5.82 & 5.60 & 5.68 & 5.66 & 5.42 & 5.46\\
\midrule\multicolumn{7}{l}{Wald}\\\midrule
\addlinespace
400 & 8.26 & 11.44 & 10.26 & 8.68 & 13.52 & 9.98\\
600 & 7.58 & 9.12 & 9.74 & 6.82 & 11.68 & 9.94\\
800 & 7.20 & 8.96 & 12.54 & 6.16 & 9.60 & 11.48\\
\bottomrule
\end{tabular}


==> size_1i_linear.tex <==

\begin{tabular}{rrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Linear - Linear} \\
\cmidrule(l{3pt}r{3pt}){3-6}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{AR} & \multicolumn{3}{c}{$\psi$} \\
\cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-6}
$n$ & $j$ &  & $k=3$ & AIC & BIC\\
\midrule
200 & 1 & 5.52 & 6.16 & 5.82 & 6.16\\
200 & 2 & 5.52 & 8.08 & 7.84 & 8.08\\
200 & 3 & 5.52 & 8.98 & 8.58 & 8.98\\
\addlinespace
400 & 1 & 5.60 & 5.80 & 5.74 & 5.80\\
400 & 2 & 5.60 & 8.20 & 8.32 & 8.20\\
400 & 3 & 5.60 & 6.62 & 6.62 & 6.62\\
\addlinespace
600 & 1 & 5.38 & 5.24 & 5.28 & 5.24\\
600 & 2 & 5.38 & 7.04 & 6.98 & 7.04\\
600 & 3 & 5.38 & 3.54 & 4.36 & 3.54\\
\bottomrule
\end{tabular}


==> size_1ii_linear.tex <==

\begin{tabular}{rlrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Linear - Linear} \\
\cmidrule(l{3pt}r{3pt}){3-6}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{AR} & \multicolumn{3}{c}{$\psi$} \\
\cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-6}
$n$ & $j_1-j_2$ &  & $k=3$ & AIC & BIC\\
\midrule
200 & 1 - 3 & 5.52 & 6.76 & 6.44 & 6.76\\
200 & 2 - 3 & 5.52 & 8.86 & 8.54 & 8.86\\
200 & 3 - 3 & 5.52 & 8.98 & 8.58 & 8.98\\
\addlinespace
400 & 1 - 3 & 5.60 & 6.36 & 6.52 & 6.36\\
400 & 2 - 3 & 5.60 & 7.96 & 7.92 & 7.96\\
400 & 3 - 3 & 5.60 & 6.62 & 6.62 & 6.62\\
\addlinespace
600 & 1 - 3 & 5.38 & 5.34 & 5.54 & 5.34\\
600 & 2 - 3 & 5.38 & 5.06 & 5.28 & 5.06\\
600 & 3 - 3 & 5.38 & 3.54 & 4.36 & 3.54\\
\bottomrule
\end{tabular}


==> size_2.tex <==

\begin{tabular}{rrrrrrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{AR} & \multicolumn{1}{c}{LM} & \multicolumn{1}{c}{CLR} & \multicolumn{1}{c}{MS$_1$} & \multicolumn{1}{c}{MS$_2$} & \multicolumn{3}{c}{$\psi$} \\
\cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7} \cmidrule(l{3pt}r{3pt}){8-10}
$n$ & $j$ &  &  &  &  &  & $k=3$ & AIC & BIC\\
\midrule
200 & 1 & 6.48 & 5.10 & 6.58 & 7.54 & 9.78 & 4.58 & 4.58 & 4.58\\
200 & 2 & 6.48 & 5.32 & 6.54 & 7.54 & 9.78 & 5.10 & 5.16 & 5.10\\
200 & 3 & 6.48 & 5.60 & 6.50 & 7.54 & 9.78 & 3.30 & 3.38 & 3.30\\
\addlinespace
400 & 1 & 6.94 & 5.48 & 6.40 & 7.50 & 8.36 & 4.80 & 4.78 & 4.80\\
400 & 2 & 6.94 & 5.52 & 6.54 & 7.50 & 8.36 & 4.62 & 4.70 & 4.62\\
400 & 3 & 6.94 & 5.92 & 6.50 & 7.50 & 8.36 & 2.16 & 2.20 & 2.16\\
\addlinespace
600 & 1 & 6.58 & 5.04 & 6.50 & 7.12 & 7.80 & 4.66 & 4.64 & 4.66\\
600 & 2 & 6.58 & 5.10 & 6.44 & 7.12 & 7.80 & 4.78 & 4.76 & 4.78\\
600 & 3 & 6.58 & 5.10 & 6.10 & 7.12 & 7.80 & 1.22 & 1.30 & 1.22\\
\bottomrule
\end{tabular}


==> size_2_linear-linear.tex <==

\begin{tabular}{rrrrrrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{AR} & \multicolumn{1}{c}{LM} & \multicolumn{1}{c}{CLR} & \multicolumn{1}{c}{MS$_1$} & \multicolumn{1}{c}{MS$_2$} & \multicolumn{3}{c}{$\psi$} \\
\cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7} \cmidrule(l{3pt}r{3pt}){8-10}
$n$ & $j$ &  &  &  &  &  & $k=3$ & AIC & BIC\\
\midrule
200 & 1 & 5.68 & 5.90 & 7.26 & 7.56 & 9.24 & 6.48 & 6.42 & 6.48\\
200 & 2 & 5.68 & 5.94 & 7.12 & 7.56 & 9.24 & 7.64 & 7.78 & 7.64\\
200 & 3 & 5.68 & 5.68 & 6.16 & 7.56 & 9.24 & 7.38 & 7.56 & 7.38\\
\addlinespace
400 & 1 & 5.28 & 4.82 & 6.28 & 7.18 & 8.78 & 5.64 & 5.70 & 5.64\\
400 & 2 & 5.28 & 5.02 & 6.06 & 7.18 & 8.78 & 4.32 & 4.46 & 4.32\\
400 & 3 & 5.28 & 4.82 & 5.42 & 7.18 & 8.78 & 2.40 & 2.68 & 2.40\\
\addlinespace
600 & 1 & 5.86 & 5.20 & 6.34 & 7.58 & 7.92 & 5.48 & 5.42 & 5.48\\
600 & 2 & 5.86 & 5.04 & 6.26 & 7.58 & 7.92 & 3.16 & 3.40 & 3.16\\
600 & 3 & 5.86 & 4.92 & 5.88 & 7.58 & 7.92 & 0.86 & 1.12 & 0.86\\
\bottomrule
\end{tabular}

